BRIGHT: A Realistic and Challenging Benchmark for Reasoning-Intensive Retrieval

Existing retrieval benchmarks primarily consist of information-seeking queries (e.g., aggregated questions from search engines) where keyword or semantic-based retrieval is usually sufficient. However, many complex real-world queries require in-depth reasoning to identify relevant documents that go beyond surface form matching. For example, finding documentation for a coding question requires understanding the logic and syntax of the functions involved. To better benchmark retrieval on such challenging queries, we introduce BRIGHT, the first text retrieval benchmark that requires intensive reasoning to retrieve relevant documents. Our dataset consists of 1,384 real-world queries spanning diverse domains, such as economics, psychology, mathematics, and coding. These queries are drawn from naturally occurring and carefully curated human data. Extensive evaluation reveals that even state-of-the-art retrieval models perform poorly on BRIGHT. The leading model on the MTEB leaderboard (Muennighoff et al., 2023) SFR-Embedding-Mistral (Meng et al., 2024), which achieves a score of 59.0 nDCG@10,1 produces a score of nDCG@10 of 18.3 on BRIGHT. We show that incorporating explicit reasoning about the query improves retrieval performance by up to 12.2 points. Moreover, incorporating retrieved documents from the top-performing retriever boosts question-answering performance. We believe that BRIGHT paves the way for future research on retrieval systems in more realistic and challenging settings.

==> tables/compare.tex <==
% \begin{table}[htbp]
% \caption{Data statistics of \ours. For each dataset, we show the number of examples, level 1 and level 2 document count, the average number of level 1 and level 2 gold documents for each example, the average length of level 1 and level 2 documents, and the average query length.}
% \centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{l|ccccccccccc}
% \toprule
%  & Sus. & Econ. & Psy. & Rob. & Earth. & Bio. & Stack. & Pony & Theo. & Math & Leet. \\
% \midrule
% \# Example & 108 & 103 & 101 & 101 & 118 & 103 & 117 & 112 \\
% \# $L1$ doc & 558 & 516 & 512 & 508 & 606 & 525 & 1862 & 577\\
% \# $L2$ doc & 60k & 50k & 52k & 62k & 122k & 57k & 107k & 7k\\
% \# $L1$ gold & 1.2 & 1.1 & 1.1 & 1.0 & 1.6 & 1.3 & 1.1 & 6.9\\
% \# $L2$ gold & 5.6 & 8.0 & 7.3 & 5.5 & 7.7 & 3.6 & 7.0 & 22.5\\
% Avg $L1$ doc len & 11k & 11k & 12k & 14k & 27k & 9k & 40k & 1k\\
% Avg $L2$ doc len & 108.0 & 120.2 & 118.2 & 120.6 & 132.4 & 83.6 & 704.5 & 98.3\\
% Avg Query len & 148.5 & 181.5 & 149.6 & 818.9 & 113.3 & 115.2 & 478.3 & 102.6\\
% \bottomrule
% \end{tabular}
% }
% \label{tab:data}
% \end{table}

\begin{table}[htbp]
\caption{
    Comparison between \ours and previous benchmarks
}
\centering
% \resizebox{\textwidth}{!}{
\begin{tabular}{c|c|c|c}
\toprule
& Query & Document & Reasoning \\
\midrule
BEIR & Claim, Title, Question & Arguments, questions, articles, tweets & \color{red}\ding{55}\\
\midrule
BIRCO & Argument
\midrule
\ours & \begin{tabular}{@{}c@{}}StackExchange post, \\ code/math questions\end{tabular} & \begin{tabular}{@{}c@{}}Examples, general web pages: news, \\ blogs, documentation, etc.\end{tabular} & \color{green}\ding{52}\\
\bottomrule
\end{tabular}
% }
\label{tab:compare}
\end{table}

==> tables/data_examples/economics_deprecated.tex <==
\begin{table}[ht]
\caption{\textbf{\econ example}}
\centering
% \resizebox{\textwidth}{!}{
\begin{tabular}{p{13cm}}
\toprule
% \hspace{5.5cm} \econ \\
% \midrule
\textit{\textbf{Query}} \\
\midrule
Would a GDP measure be improved by excluding foreign interest paid? \\
The income method of calculating GDP is as follows: GDP = wages + profits + rents + interest + depreciation + taxes + NFFI. If an economy has high external debt, for instance, because it used external financing to buy machinery and equipment, then foreign interest payments will be high. In that case, wouldn't GDP (per capita) be a poor measure of economic well-being since a significant portion of the generated income is leaving the home economy? \\
Wouldn't excluding foreign interest payments in calculating GDP/ income give us a better measure since this represents what income is available to the home economy? \\
\midrule
\textit{\textbf{Reasoning steps}} \\
\midrule
The statement implies that GDP serves as an indicator of economic well-being, yet GDP, Gross domestic product,  primarily reflects economic production and outputs rather than directly gauging well-being. It's crucial to understand the association between GDP and economic well-being. \\
\midrule
\textit{\textbf{Example positive document}} \\
\midrule
Measuring well-being is about going beyond the cold numbers of GDP. But cold as it may be, GDP remains a very important indicator for measuring the economic performance of countries, which is a fundamental driver of well-being. This is not only because income means higher material standards but also because income is needed to sustain private and public spending in non-material components of well-being, such as education and health. However, there is an increasing recognition that focusing on GDP alone is not enough to achieve better lives for all. \\
The relationship between a country’s s GDP per capita and well-being is usually positive – in other words, countries with higher GDP per capita are also those where well-being is higher on average. However this relationship becomes weaker as a country’s income grows, suggesting that once income reaches a certain level, increased income is less likely to generate well-being. The other interesting phenomenon is that some countries do better at delivering wellbeing than they do if gauged only on the basis of economic production per capita. This is the case for Nordic European countries but also for New Zealand. On the other hand,  there are countries that do better in GDP per capita than on average well-being,  for instance the United States and Switzerland. \\
% So why in these two sets of countries do economic performance and well-being  not go strictly  hand in hand? One explanation is that the countries that do better in terms of well-being have  made the choice of working less to achieve a better work and life balance. This translates into lower income but also increased leisure time that can be shared with friends and family, or that is used for volunteering and engaging with the community. Another reason is that these countries have better environmental quality, partly because of lower economic production and thus pollution. Well-being is a matter of democracy and societal choices, what really matters at the end of the day is whether countries are where their citizens would like them to be. It can be higher economic production or more time for life, longer healthy lives or more connected neighbourhoods. What is important is to collect the relevant set of statistics to judge whether collective objectives are met and ensure that governments are paying the right degree of attention to these statistics.\\
... \\
\midrule
\textit{\textbf{Example negative document}} \\
\midrule
The impact of foreign interest rates on the economy: The role of the exchange rate regime\\
It is often argued that many economies are affected by conditions in foreign countries. This paper explores the connection
between interest rates in major industrial countries and annual real output growth in other countries. The results show that high
foreign interest rates have a contractionary effect on annual real GDP growth in the domestic economy, but that this effect is
centered on countries with fixed exchange rates. The paper then examines the potential channels through which major-country
interest rates affect other economies. The effect of foreign interest rates on domestic interest rates is the most likely channel when
compared with other possibilities, such as a trade effect. \\
... \\
This paper answers two questions. First, what is the effect of interest rates in base countries on other countries' annual
real GDP growth?3 Second, how does this effect vary by the exchange rate regime and other country characteristics?
Answering the second question helps to disentangle the channels through which foreign country interest rates affect
other economies. We find that annual real output growth in countries is negatively associated with interest rates in their
base countries, but that this effect holds only for countries with fixed exchange rates. \\
... \\
\bottomrule
\end{tabular}
% }
\label{tab:economic_example}
\end{table}

==> tables/main_results_howard.tex <==
\begin{table}[htbp]
    \caption{Retrieval performance. We report nDCG@10 for all datasets except nDCG@50 for Pony. The datasets are: Sus.--Sustainable Living; Econ.--Economics; Psy.--Psychology \& Neuroscience; Rob.--Robotics; Earth.--Earth Science; Bio.--Biology; Stack.--Stack Overflow; Theo.--TheoremQA; Leet.--Leetcode. The average performance of all models are no more than 20, indicating the challenge of \ours to current models.\todo{split the open-sourced models into available weights and available code.}}
    \centering
    \resizebox{\textwidth}{!}{
        \begin{tabular}{l|ccccccccccc|c}
            \toprule
            & Sus. & Econ. & Psy. & Rob. & Earth. & Bio. & Stack. & Pony & Theo. & MATH & Leet. & Avg. \\
            \midrule
            \multicolumn{13}{c}{Sparse model} \\
            \midrule
            BM25 & 15.2 & 14.9 & 12.5 & 13.5 & 27.1 & 19.2 & 16.5 & 11.6 & 6.9 & 10.4 & 24.4 & 15.7 \\
            \midrule
            \multicolumn{13}{c}{Open-sourced models (<1B)} \\
            \midrule
            SBERT & 15.0 & 16.7 & 22.4 & 8.3 & 20.0 & 15.7 & 9.3 & 9.3 & 13.2 & 14.0 & 26.3 & 15.5 \\
            BGE & 12.8 & 16.6 & 17.2 & 12.1 & 24.2 & 12.1 & 9.3 & 9.6 & 9.0 & 11.9 & 26.8 & 14.7 \\
            Inst-L & 13.3 & 14.3 & 19.8 & 9.4 & 22.2 & 16.0 & 9.1 & 2.9 & 13.5 & 13.7 & 20.4 & 14.1 \\
            \midrule
            \multicolumn{13}{c}{Open-sourced models (>1B)} \\
            \midrule
            Inst-XL & 18.5 & 20.2 & 25.1 & 15.1 & 32.2 & 21.2 & 15.1 & 7.0 & 11.5 & 13.8 & 28.6 & 18.9 \\
            Qwen & 21.7 & 17.3 & 23.6 & 13.0 & 39.0 & 31.2 & 19.3 & 11.3 & 14.6 & 16.0 & 25.9 & 21.2 \\
            E5 & 18.5 & 15.5 & 15.7 & 16.9 & 26.1 & 18.6 & 9.9 & 12.3 & 16.4 & 14.1 & 28.5 & 17.5 \\
            Grit & 7.9 & 18.6 & 19.8 & 17.2 & 33.1 & 7.5 & 10.5 & 21.5 & 15.3 & 15.0 & 29.6 & 17.8 \\
            SFR & 19.2 & 18.2 & 19.7 & 17.6 & 26.6 & 20.0 & 11.8 & 10.6 & 16.2 & 15.3 & 27.7 & 18.4 \\
            \midrule
            \multicolumn{13}{c}{Proprietary models} \\
            \midrule
            Cohere &  &  &  &  &  &  &  &  & 10.9 & 12.2 & 27.0 &  \\
            OpenAI &  &  &  &  &  &  &  &  & 16.3 & 14.0 & 26.5 &  \\
            Voyage &  &  &  &  &  &  &  &  & 18.1 & 13.9 & 30.6 & \\
            Google &  &  &  &  &  &  &  &  & & & & \\
            \bottomrule
        \end{tabular}
    }
    \label{tab:main_results}
\end{table}

==> tables/qa_gpt4.tex <==
\begin{table}
\centering

\caption{\textbf{Question answering results with different retrievers.}
We use the GPT-4 as the generation models, and evaluate the answers with Claude-3.5-sonnet.
Results show that stronger retrieval typically result in better QA results, indicating the helpfulness of the annotated documents for addressing the posts in StackExchange.
}
\label{tab:qa_gpt4}
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{l|ccccccc|c}
\toprule
 \textbf{Retriever} & \textbf{Bio.} & \textbf{Earth.} & \textbf{Econ.} & \textbf{Psy.} & \textbf{Rob.} & \textbf{Stack.} & \textbf{Sus.} & \textbf{Average} \\
\midrule
None & 62.6 & 64.9 & 57.8 & 58.2 & 53.5 & 64.4 & 49.8 & 58.7 \\
\midrule
\bmtwentyfive & 64.3 & 65.2 & 57.8 & 54.6 & 60.2 & 65.9 & 56.5 & 60.6 \\
\sentencebert & 62.2 & 63.2 & 59.7 & 65.6 & 55.7 & 59.9 & \textbf{61.0} & 61.0 \\
\qwen & \textbf{69.4} & \textbf{68.3} & \textbf{62.0} & \textbf{66.3} & \textbf{64.2} & \textbf{69.5} & 55.5 & \textbf{65.0} \\
\midrule
Oracle & \textit{80.0} & \textit{81.2} & \textit{73.6} & \textit{77.8} & \textit{70.5} & \textit{80.4} & \textit{70.6} & \textit{76.3} \\
\bottomrule
\end{tabular}
}
\end{table}

==> tables/reason.tex <==
\begin{table}[htbp]
\caption{Detailed scores of retrieval models when using LLM reasoning steps as queries.}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{l|ccccccccccc|c}
\toprule
 & Sus. & Econ. & Psy. & Rob. & Earth. & Bio. & Stack. & Pony & Theo. & Math & Leet. & Avg. \\
\midrule
\multicolumn{13}{c}{Sparse models} \\
\midrule
BM25 & 11.1 & 13.4 & 15.8 & 5.3 & 10.2 & 17.5 & 8.4 & 1.6 & & & & 10.4\\
\midrule
\multicolumn{13}{c}{Open-sourced models (<1B)} \\
\midrule
SBert & 15.2 & 18.0 & 27.5 & 12.1 & 21.9 & 20.8 & 12.4 & 6.2 & & & & 16.8\\
BGE & 17.4 & 22.8 & 22.9 & 13.5 & 29.9 & 21.3 & 12.5 & 4.0 & & & & 18.0\\
I-large & 15.5 & 23.3 & 29.6 & 16.2 & 29.1 & 28.4 & 13.1 & 2.6 & & & & 19.7\\
\midrule
\multicolumn{13}{c}{Open-sourced models (>1B)} \\
\midrule
I-xl & 25.2 & 28.2 & 35.5 & 20.2 & 34.3 & 37.3 & 18.5 & 4.4 & & & & 25.4\\
Qwen & 19.7 & 19.6 & 20.8 & 14.2 & 24.6 & 21.8 & 14.7 & 15.2 & & & & 18.8\\
E5 & 15.1 & 21.5 & 22.5 & 16.5 & 38.3 & 27.4 & 14.8 & 0.3 & & & & 19.5\\
Grit & 13.6 & 23.4 & 24.7 & 18.2 & 26.9 & 20.1 & 12.4 & 7.0 & & & & 18.3\\
SFR & 17.0 & 23.6 & 25.9 & 17.5 & 34.5 & 24.4 & 15.4 & 0.4 & & & & 19.8\\
\bottomrule
\end{tabular}
}
\label{tab:reason}
\end{table}

==> tables/rerank/qwen.tex <==
\begin{table}[htbp]
\caption{\textbf{\minilm (cross-encoder), Gemini and GPT-4 reranking scores based on \qwen retrieval top-10 or top-100 results.} We also include the retrieval results (reranker=None) for easier reference.
}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lc|ccccccc|cc|ccc|c}
\toprule
 & & \multicolumn{7}{c|}{StackExchange} & \multicolumn{2}{c|}{Code} & \multicolumn{3}{c|}{Math} & \multirow{2}{*}{\centering Avg.}\\
\cmidrule(r){3-9} \cmidrule(r){10-11} \cmidrule(r){12-14}
Reranker & top-k & Bio. & Earth. & Econ. & Psy. & Rob. & Stack. & Sus. & Leet. & \pony  & \aops & TheoQ. & TheoT. \\
\midrule
None & - & 30.9 & 36.2 & 17.7 & 24.6 & 13.5 & 19.9 & 14.9 & 25.5 & 9.8 & 14.4 & 27.0 & 26.7 & 21.7 \\
\midrule
\multirow{2}{*}{\centering \minilm} & 10 &  \\
& 100 &  \\
\midrule
Gemini & 10 & 33.3 & 37.1 & 18.2 & 25.7 & 14.7 & 20.2 & 15.4 & 25.2 & 11.2 & 14.4 & 25.9 & 26.5 & 22.3 \\
\midrule
\multirow{2}{*}{\centering GPT-4} & \\
 & 100 & \\
\bottomrule
\end{tabular}
}
\label{tab:results_rerank_qwen}
\end{table}

==> texts/ack.tex <==
\begin{ack}
We thank Qilin Liao, Yun Han, Xiaoru Teng, Cong Gao, Shengyu Wang, Xiaodong Wei, and Yan Pan for annotating and reviewing the datasets.
We would also like to thank Kenny Huang for his helpful discussions on collecting data from the \aops Wiki.
\end{ack}

==> texts/appendices/case_study.tex <==
\section{Case Study: Retrieving Relevant Examples Improves Model Performance}
\label{sec:case_study}
\ours is designed to meet users' needs to retrieve documents that are intrinsically relevant to the query beyond simple semantic matching. Besides serving users with retrieved documents, these documents can also be used as context for language models to provide an answer to the query directly, known as retrieval augmented generation (RAG). While our work focuses on evaluating retrieval performance, we also provide a case study in the RAG setting. This illustrates how annotated documents from \ours can enhance the performance of language models to solve the query, whereas documents retrieved from state-of-the-art retrieval systems fail to do so. 

We present an example from the \theorem dataset, where the query is a math problem that essentially requires using an integral rule to derive the original form of the function. 
Our gold positive example features a similar problem utilizing the same theorem. 
With this gold example as context, our model---\ttt{gpt-4-0125-preview}---successfully derives the correct solution, despite the surface differences between the gold positive example and the query. 
In contrast, the random example and the examples retrieved by BM25 and Qwen do not require the use of the integral rule; instead, they feature algebraic and combinatoric problems, respectively. 
With the retrieved example in the context, the model fails to derive the correct solution. 
This case study demonstrates that our gold annotation also has the potential to improve RAG performance by providing relevant examples. 
We will leave a systematic evaluation of RAG for future work. 



\begin{example}[Query (a math problem from \theorem)]
\begin{lstlisting}
You're tracking the growth of a plant from a seed. The rate at which 
the plant grows in height is equal to the square root of the number 
of days since you planted it. One day after the seed was first 
planted, the plant was 1 inch tall. How tall will the plant be after 
4 days?
  \end{lstlisting}
\end{example}
\begin{correctanswer}
\small{\textbf{Gold Positive Example}: 
  ${\frac{dy}{dx}} = \sqrt{t}, y(1) = 1$. What is $y(16)$?\newline\newline
  To find $y(4)$, we need to solve the given differential equation and apply the initial condition $y(1) = 1$.\newline
  The given differential equation is: ${\frac{dy}{dx}} = \sqrt{t}$\newline
  To solve this, we can integrate both sides with respect to $t$:\newline
  $\int dy = \int \sqrt{t} \, dt$\newline
  $y(t) = (2/3)t^{(3/2)} + C$ \newline
  Now, we apply the initial condition $y(1) = 1$: \newline
  $1 = (2/3)(1)^{(3/2)} + C$\newline
  $1 = 2/3 + C$\newline
  $C = 1/3$\newline
  So, the solution to the differential equation is: $y(t) = (2/3)t^{(3/2)} + 1/3$\newline
  Now, we can find $y(16)$:\newline
  $y(4) = (2/3)(16)^{(3/2)} + 1/3$\newline
  $y(4) = (2/3)(64) + 1/3$\newline
  $y(4) = 128/3 + 1/3$\newline
  $y(4) = 43$\newline
  Therefore, the answer is $43$.\newline
  }

  \small{\textbf{Model Output \cmark}: The growth rate of the plant is given by the differential equation $\frac{dy}{dx} = \sqrt{t}$, with the initial condition $y(1) = 1$, which is exactly the same as the differential equation problem described above. Therefore, the solution process and the final solution apply here as well. We found that $y(t) = (2/3)t^(3/2) + 1/3$. To find the height of the plant after 4 days, we substitute $t = 4$ into this equation.\newline
  $y(4) = (2/3)(4)^(3/2) + 1/3 = 17/3$\newline
  Therefore, the plant will be 17/3 inches tall after 4 days. }
\end{correctanswer}

\begin{wronganswer}
\label{fig:random_example}
\small{\textbf{Random Example}: What is the smallest positive integer that can be multiplied by 605 to make it a perfect square?Answer Choices: (A) 2 (B) 3 (C) 5 (D) 7 (E) 11\newline\newline
Let's reason about the multi-choice question.\newline
605 is multiplied by 5 gives 3025\newline
Its a square root of 55\newline
The answer is 5 -Option C\newline}

\textbf{Model Output \xmark}: \small{The growth rate of the plant is equal to the square root of the number of days since it was planted. After 4 days, the height of the plant will be equal to the square root of 4, which is 2. Therefore, the plant will be 2 inches tall after 4 days.}
\end{wronganswer}

\begin{wronganswer}
\small{\textbf{BM25 Example}: A basketball team has 12 players, including 5 guards and 7 forwards. How many different starting lineups can be formed that include 3 guards and 2 forwards?\newline\newline
To form a starting lineup with 3 guards and 2 forwards, we need to choose 3 guards from the 5 available guards and 2 forwards from the 7 available forwards. We can use the combination formula to calculate this:\newline
Number of ways to choose 3 guards from 5 $= C(5, 3) = 5! / (3! * (5-3)!) = 10$\newline
Number of ways to choose 2 forwards from 7 $= C(7, 2) = 7! / (2! * (7-2)!) = 21$\newline
Now, we multiply the number of ways to choose guards and forwards to get the total number of different starting lineups:\newline
Total starting lineups = 10 (ways to choose guards) * 21 (ways to choose forwards) = 210\newline
Therefore, the answer is 210.\newline
}

\textbf{Model Output \xmark}: \small{To find the height of the plant after 4 days, we use the given rate of growth: the square root of the number of days since the plant was planted. Since the height of the plant is equal to the square root of the number of days, we just substitute 4 days into the formula:\newline
Height after 4 days = sqrt(4) = 2 inches.\newline
Thus, the plant will be 2 inches tall after 4 days.
}
\end{wronganswer}

\begin{wronganswer}
\label{fig:qwen_example}
 \small{\textbf{Qwen Example}: A basketball team has 10 players, but only 5 can play at a time. In how many ways can the coach choose the 5 players who will play in the starting lineup?\newline\newline
To determine the number of ways the coach can choose the 5 players for the starting lineup, we can use the combination formula. The combination formula is:\newline
$C(n, k) = n! / (k!(n-k)!)$\newline
where n is the total number of players (10 in this case), k is the number of players to choose (5 in this case), and ! denotes the factorial function $(e.g., 5! = 5 × 4 × 3 × 2 × 1)$.\newline
So, we have:\newline
$C(10, 5) = 10! / (5!(10-5)!)$\newline
$C(10, 5) = 10! / (5!5!)$\newline
Now, let's calculate the factorials:
$10! = 10 × 9 × 8 × 7 × 6 × 5 × 4 × 3 × 2 × 1 = 3,628,800$\newline
$5! = 5 × 4 × 3 × 2 × 1 = 120$\newline}

\small{\textbf{Model Output \xmark}: To determine the height of the plant after 4 days, we use the given growth rate formula: the height of the plant is equal to the square root of the number of days since it was planted.\newline
On day 1, the plant is 1 inch tall, which is consistent with the formula since the square root of 1 is 1.\newline
To find out the height after 4 days, we substitute the number of days (4) into the square root formula:\newline
Height $ = \sqrt{\text{days}} = \sqrt{4}$\newline
The square root of 4 is 2.\newline
Thus, the plant will be 2 inches tall after 4 days.
}

\end{wronganswer}


==> texts/appendices/datadoc.tex <==
BRIGHT is the first text retrieval benchmark that requires intensive reasoning to retrieve relevant documents. The queries are collected from diverse domains (StackExchange, LeetCode, and math competitions), all sourced from realistic human data. Experiments show that existing retrieval models perform poorly on BRIGHT, where the highest score is only 21 measured by nDCG@10. BRIGHT provides a good testbed for future retrieval research in more realistic and challenging settings.

\paragraph{Data Card Author(s)}
\begin{itemize}
    \item \textbf{Hongjin Su, HKU:} Owner
    \item \textbf{Howard Yen, Princeton:} Owner
    \item \textbf{Mengzhou Xia, Princeton:} Owner
    \item \textbf{Weijia Shi, UW:} Contributor
    \item \textbf{Niklas Muennighoff:} Contributor
    \item \textbf{Han-yu Wang, HKU:} Contributor
    \item \textbf{Haisu Liu, HKU:} Contributor
    \item \textbf{Quan Shi, Princeton:} Contributor
    \item \textbf{Zachary S. Siegel, Princeton:} Contributor
    \item \textbf{Michael Tang, Princeton:} Contributor
    \item \textbf{Ruoxi Sun, Google:} Contributor
    \item \textbf{Jinsung Yoon, Google:} Contributor
    \item \textbf{Sercan Ö. Arik, Google:} Contributor
    \item \textbf{Danqi Chen, Princeton:} Contributor
    \item \textbf{Tao Yu, HKU:} Contributor
\end{itemize}

\subsection{Authorship}

\subsubsection{Publishers}

\paragraph{Publishing Organization(s)}
The University of Hong Kong

\paragraph{Industry Type(s)}
\begin{itemize}
    \item Academic - Tech
\end{itemize}

\paragraph{Contact Detail(s)}
\begin{itemize}
    \item \textbf{Publishing POC:} N/A
    \item \textbf{Affiliation:} N/A
    \item \textbf{Contact:} N/A
    \item \textbf{Mailing List:} N/A
    \item \textbf{Website:} N/A
\end{itemize}

\subsubsection{Dataset Owners}

\paragraph{Team(s)}
Hongjin Su, Howard Yen, and Mengzhou Xia

\paragraph{Contact Detail(s)}
\begin{itemize}
    \item \textbf{Dataset Owner(s):} Hongjin Su, Howard Yen, and Mengzhou Xia
    \item \textbf{Affiliation:} The University of Hong Kong and Princeton University
    \item \textbf{Contact:} hjsu@cs.hku.hk, \{hyen, mengzhou\}@cs.princeton.edu
    \item \textbf{Group Email:} N/A
    \item \textbf{Website:} N/A
\end{itemize}

\paragraph{Author(s)}
\begin{itemize}
    \item Hongjin Su, PhD student, The University of Hong Kong
    \item Howard Yen, Masters student, Princeton University
    \item Mengzhou Xia, PhD student, Princeton University
\end{itemize}

\subsubsection{Funding Sources}

\paragraph{Institution(s)}
\begin{itemize}
    \item Princeton University
    \item Google Cloud AI Research
\end{itemize}

\paragraph{Funding or Grant Summary(ies)}
We thank the Princeton University and Google Cloud AI Research for supporting Nvidia GPUs to benchmark retrieval models on BRIGHT.

\subsection{Dataset Overview}

\subsubsection{Data Subject(s)}
\begin{itemize}
    \item Non-Sensitive Data about people
    \item Public data accessible to everyone
\end{itemize}

\subsubsection{Dataset Snapshot}

\begin{tabular}{|l|l|}
\hline
Category & Data \\
\hline
Size of Dataset & 607 MB \\
Number of Instances & 1322 \\
Number of Fields & 6 \\
Domains & 11 \\
\hline
\end{tabular}

\textbf{Above:} We collect 1322 diverse queries from realistic human data. Each example is annotated with the gold documents and the reasoning traces to find them.

\subsubsection{Content Description}
The datasets are collected from \href{https://stackexchange.com/}{StackExchange}, \href{https://arxiv.org/abs/2305.12524}{TheoremQA}, \href{https://leetcode.com/}{LeetCode}, and \href{https://artofproblemsolving.com/}{Math competition}.

\subsubsection{Descriptive Statistics}

\begin{tabular}{|l|l|l|l|l|l|}
\hline
Dataset & \# Q & \# D & \# D+ & Q.L. & D.L. \\
\hline
Biology & 103 & 57,364 & 3.6 & 83.6 & 115.2 \\
Earth Science & 118 & 122,388 & 7.7 & 132.4 & 113.3 \\
Economics & 103 & 50,221 & 8.0 & 120.2 & 181.5 \\
Psychology & 101 & 52,841 & 7.3 & 118.2 & 149.6 \\
Robotics & 101 & 62,198 & 5.5 & 120.6 & 818.9 \\
Stack Overflow & 117 & 101,100 & 7.0 & 704.5 & 478.3 \\
Sustainable Living & 108 & 60,732 & 5.6 & 108.0 & 148.5 \\
LeetCode & 142 & 413,932 & 1.8 & 483.1 & 497.5 \\
Pony & 112 & 7,894 & 22.5 & 98.3 & 102.6 \\
AoPS & 111 & 188,177 & 4.7 & 89.0 & 250.5 \\
TheoremQA & 206 & 188,177 & 3.2 & 117.1 & 250.5 \\
\hline
\end{tabular}

Data statistics of BRIGHT. For each dataset, we show the number of queries (\# Q) and documents (\# D), the average number of positive documents (\# D+) per example, the average length of queries (Q.L.) and documents (D.L., measured by the GPT-2 tokenizer).

\subsubsection{Sensitivity of Data}

\paragraph{Sensitivity Type(s)}
\begin{itemize}
    \item None
\end{itemize}

\paragraph{Field(s) with Sensitive Data}
\begin{itemize}
    \item None
\end{itemize}

\paragraph{Security and Privacy Handling}
We select academia-oriented domains and remove all user information in StackExchange data.

\paragraph{Risk Type(s)}
\begin{itemize}
    \item No Known Risks
\end{itemize}

\paragraph{Supplemental Link(s)}
\begin{itemize}
    \item None
\end{itemize}

\paragraph{Risk(s) and Mitigation(s)}
\begin{itemize}
    \item N/A
\end{itemize}

\subsubsection{Dataset Version and Maintenance}

\paragraph{Maintenance Status}
\textbf{Actively Maintained} - No new versions will be made available, but this dataset will be actively maintained, including but not limited to updates to the data.

\paragraph{Version Details}
\begin{itemize}
    \item \textbf{Current Version:} 1.0
    \item \textbf{Last Updated:} 06/2024
    \item \textbf{Release Date:} 06/2024
\end{itemize}

\paragraph{Maintenance Plan}
We will mainly use Github issues and HuggingFace communities to address any issues the users encounter in using the BRIGHT data.

\textbf{Versioning:} If new versions are released, it will become 1.1 or 2.0 depending on the update.

\textbf{Updates:} There may be updates in the future.

\textbf{Errors:} We will address the errors users encounter.

\textbf{Feedback:} Either by email, Github issue, or HuggingFace community, we welcome all feedback to make this benchmark better.

\paragraph{Next Planned Update(s)}
\begin{itemize}
    \item \textbf{Version affected:} N/A
    \item \textbf{Next data update:} N/A
    \item \textbf{Next version:} N/A
    \item \textbf{Next version update:} N/A
\end{itemize}

\paragraph{Expected Change(s)}
\textbf{Updates to Data:} N/A

\textbf{Updates to Dataset:} N/A

\subsection{Example of Data Points}

\subsubsection{Primary Data Modality}
\begin{itemize}
    \item Text Data
\end{itemize}

\subsubsection{Sampling of Data Points}
\href{https://huggingface.co/datasets/xlangai/BRIGHT/blob/main/data_examples.pdf}{Typical Data Points Link}

\subsubsection{Typical Data Point}
Summarize here. Include any criteria for typicality of data point.

\begin{lstlisting}[breaklines]
  "query": "Claim in article about why insects are attracted to light\nIn this
  article they are addressing the reason insects are attracted to light when they say\nHeat radiation as an attractive component is refuted by the effect of LED lighting, which supplies negligible infrared radiation yet still entraps vast numbers of insects.\nI don't see why attraction to LEDs shows they're not seeking heat. Could they for example be evolutionarily programmed to associate light with heat? So that even though they don't encounter heat near/on the LEDs they still 'expect' to?",
  "reasoning": "The question probes why insects are drawn to low-heat LED lights, challenging the idea that their attraction to light is heat-based. The document helps distinguish between heat attraction and evolved behaviors, shedding light on why insects might be attracted to LEDs despite their minimal heat.",
  "id": "0",
  "excluded_ids": [
    "N/A"
  ],
  "gold_ids_long": [
    "insects_attracted_to_light/Proximate_and_ultimate_causation.txt",
    "insects_attracted_to_light/Phototaxis.txt"
  ],
  "gold_ids": [
    "insects_attracted_to_light/Phototaxis_3.txt",
    "insects_attracted_to_light/Proximate_and_ultimate_causation_0.txt",
    "insects_attracted_to_light/Phototaxis_4.txt",
    "insects_attracted_to_light/Proximate_and_ultimate_causation_1.txt",
    "insects_attracted_to_light/Phototaxis_0.txt"
  ]
}
\end{lstlisting}

\subsection{Motivations \& Intentions}

\subsubsection{Motivations}

\paragraph{Purpose(s)}
\begin{itemize}
    \item Research
\end{itemize}

\paragraph{Domain(s) of Application}
\texttt{retrieval}

\paragraph{Motivating Factor(s)}
\begin{itemize}
    \item Existing retrieval benchmarks can be solved by lexical or semantic match
    \item Many realistic scenarios cannot be solved by such simple match
    \item To bridge this gap, we introduce BRIGHT to evaluate retrieval models in realistic settings where intensive reasoning is required
\end{itemize}

\subsubsection{Intended Use}

\paragraph{Dataset Use(s)}
\begin{itemize}
    \item Evaluate retrieval systems in realistic scenarios
\end{itemize}

\paragraph{Suitable Use Case(s)}
\textbf{Suitable Use Case:} Evaluate retrieval models

\paragraph{Unsuitable Use Case(s)}
\textbf{Unsuitable Use Case:} Train retrieval models

\paragraph{Research and Problem Space(s)}
We investigate new directions of retrieval, where the relevance between queries and documents goes beyond lexical and semantic similarities.

\paragraph{Citation Guidelines}
\textbf{Guidelines \& Steps:} Include citation when using BRIGHT

\textbf{BiBTeX:}
\begin{lstlisting}[breaklines]
    @inproceedings{BRIGHT,
  title={BRIGHT: A Realistic and Challenging Benchmark for Reasoning-Intensive Retrieval},
  author={Su, Hongjin and Yen, Howard and Xia, Mengzhou and Shi, Weijia and Muennighoff, Niklas and Wang, Han-yu and Liu, Haisu and Shi, Quan and Siegel, Zachary S and Tang, Michael and Sun, Ruoxi and Yoon, Jinsung and Arik, Sercan O and Chen, Danqi and Yu, Tao},
  year={2024},
}
\end{lstlisting}


\subsection{Access, Rentention, \& Wipeout}
\subsubsection{Access}
\paragraph{Access Type}
% scope: telescope
% info: Select \textbf{one}:
- External - Open Access

\paragraph{Documentation Link(s)}
% scope: periscope
% info: Provide links that describe documentation to access this dataset:
- Dataset Website URL: \url{https://huggingface.co/datasets/xlangai/BRIGHT}
- GitHub URL: \url{https://github.com/xlang-ai/BRIGHT}

\paragraph{Prerequisite(s)}
% scope: microscope
% info: Please describe any required training or prerequisites to access this dataset.
N/A

\paragraph{Policy Link(s)}
% scope: periscope
% info: Provide a link to the access policy:
- Direct download URL: \url{https://huggingface.co/datasets/xlangai/BRIGHT}

Code to download data:
\begin{verbatim}
from datasets import load_dataset
data = load_dataset('xlangai/BRIGHT', 'examples')['biology']
\end{verbatim}

\paragraph{Access Control List(s)}
% scope: microscope
% info: List and summarize any access control lists associated with this dataset. Include links where necessary. Use additional notes to capture any other information relevant to accessing the dataset.
N/A

\subsubsection{Retention}
Free retention

\subsubsection{Wipeout and Deletion}
We are not currently considering wiping out or deleting the data

\subsection{Provenance}
\subsubsection{Collection}
\paragraph{Method(s) Used}
% scope: telescope
% info: Select \textbf{all applicable} methods used to collect data:
- Data are collected by authors

\paragraph{Methodology Detail(s)}
% scope: periscope
% info: Provide a description of each collection method used. Use additional notes to capture any other relevant information or considerations. (Usage Note: Duplicate and complete the following for collection method type.)
\textbf{Collection Type}

\textbf{Source:} \url{https://stackexchange.com/}, \url{https://arxiv.org/abs/2305.12524}, \url{https://leetcode.com/} and \url{https://artofproblemsolving.com/}.

\textbf{Platform:} N/A

\textbf{Is this source considered sensitive or high-risk?} No

\textbf{Dates of Collection:} 2024.03 to 2024.05

\textbf{Primary modality of collection data:}

% Usage Note: Select one for this collection type.

- Text Data

\textbf{Update Frequency for collected data:}

% Usage Note: Select one for this collection type.

- Static

\textbf{Additional Links for this collection:}

N/A

\paragraph{Source Description(s)}
\begin{itemize}
\item \textbf{Source:} StackExchange is a popular question-answering platform where users ask questions and receive answers from the community. \href{https://sustainability.stackexchange.com/questions/4691/how-good-is-it-to-reuse-water-from-plant-pots}{One example} is
\begin{lstlisting} [breaklines]
How good is it to reuse water from plant pots?
I'm living in an apartment, and after I water my plants the water goes to plates below the pots. The pots are in a metallic structure above the plates, so I can take the plates to reuse the water (throwing it at the plants again).
This reuse seems beneficial, because I think I can get rid of mosquitoes that would reproduce in the stagnated water. And also some nutrients of the soil (as well as earthworms) can return to the vase.
Is there some negative points in doing that?
EDIT: I think I must add that I'm at 3 degrees of latitude, in a hot and humid tropical rainforest, where the precipitation used to be around 1700 mm. So I use lots of water everyday, more than once a day sometimes, so the reused water is a small fraction of the water used.
waterreuseplants
Share
Improve this question
Follow
edited Mar 17, 2016 at 15:27
asked Sep 3, 2015 at 18:39
Rodrigo's user avatar
Rodrigo
16311 silver badge 66 bronze badges
i think you mean "pots" if they have dirt in them. "vases" hold water and cur flowers. - Kate Gregory Mar 17, 2016 at 14:53
Add a comment
2 Answers
Sorted by:
Highest score (default)
7
In my experience plants suffer in the long term from accumulation of salts in the soil, so fresh water would be better than reusing the water. Even better would be to get hold of fresh rain water (tricky in an apartment though, unless perhaps you have a balcony that gets rained on) for watering them, as that won't contain the salts that tap water does.
More detail here.
Share
Improve this answer
Follow
\end{lstlisting}
\item \textbf{Source:} LeetCode is a popular coding platform for programmers to practice. One example is:
\begin{lstlisting} [breaklines]
5. Longest Palindromic Substring
Medium
Topics
Companies
Hint
Given a string s, return the longest palindromic substring in s.
Example 1:
Input: s = "babad"
Output: "bab"
Explanation: "aba" is also a valid answer.
Example 2:
Input: s = "cbbd"
Output: "bb"
Constraints:
1 <= s.length <= 1000
s consist of only digits and English letters.
\end{lstlisting}

\item \textbf{Source:} \begin{lstlisting} [breaklines] AoPS contains math competition questions. [One example] is:
Problem 1
What is the ones digit of 222,22 -222,222, -2,222,-222222 
A. 0
B. 2
C. 4
D. 6
E. 8      

Solution 1
We can rewrite the expression as 222,222-(22,222+2,222+222+22+2).
We note that the units digit of the addition is 0 because all the units digits of the five numbers are 2 and 5*2=10, which has a units digit of 0.
Now, we have something with a units digit of 0 subtracted from 222,222. The units digit of this expression is obviously 2, and we get \boxed{B} as our answer.
\end{lstlisting}
\end{itemize}

\paragraph{Collection Cadence}
% scope: telescope
% info: Select \textbf{all applicable}:
\begin{itemize}
\item \textbf{Static:} Data was collected once from single or multiple sources.
\end{itemize}

\paragraph{Data Integration}
\begin{itemize}
\item \textbf{Source} N/A

\item \textbf{Included Fields} Data fields that were collected and are included in the dataset.

\begin{tabular}{|l|l|}
\hline
Field Name & Description \\
\hline
Post & The content of post where users ask questions \\
\hline
\end{tabular}

\item  \textbf{Additional Notes:} Add here

\item  \textbf{Excluded Fields} Data fields that were collected but are excluded from the dataset.

\begin{tabular}{|l|l|}
\hline
Field Name & Description \\
\hline
Answer & Community answers \\
Votes & The votes for the post of answers \\
\hline
\end{tabular}
\end{itemize}

\paragraph{Data Processing}
% scope: microscope
% info: Summarize how data from different sources or methods aggregated, processed, or connected. Use additional notes to capture any other relevant information or considerations. (Usage Note: Duplicate and complete the following for each source OR collection method.)

All the data collection and processing are done manually or with the help of python scripts.

\subsubsection{Collection Criteria}
\paragraph{Data Selection}
% scope: telescope
% info: Summarize the data selection criteria. Use additional notes to capture any other relevant information or considerations.
\begin{itemize}
\item \textbf{StackExchange:} We select posts that have links in answers receiving user accept or more than 5 votes
\item  \textbf{Math and Code:} We select questions that require a theorems of syntax documentation.
\end{itemize}

\paragraph{Data Inclusion}
% scope: periscope
% info: Summarize the data inclusion criteria. Use additional notes to capture any other relevant information or considerations.
We include data from diverse domains including psychology, robotics, etc.

\paragraph{Data Exclusion}
% scope: microscope
% info: Summarize the data exclusion criteria. Use additional notes to capture any other relevant information or considerations.
We exclude examples that do not require reasoning in retrieval or do not use theorems.

\subsubsection{Relationship to Source}
\paragraph{Use \& Utility(ies)}
% scope: telescope
% info: Describe how the resulting dataset is aligned with the purposes, motivations, or intended use of the upstream source(s). Use additional notes to capture any other relevant information or considerations. (Usage Note: Duplicate and complete the following for each source type.)
\begin{itemize}
\item \textbf{StackExchange:} We use the post and linked web pages in answers
\item \textbf{Math \& Code:} We use the questions and tags in websites.
\end{itemize}

\paragraph{Benefit and Value(s)}
% scope: periscope
% info: Summarize the benefits of the resulting dataset to its consumers, compared to the upstream source(s). Use additional notes to capture any other relevant information or considerations. (Usage Note: Duplicate and complete the following for each source type.)
- Using this method, we collect retrieval instances that require intensive reasoning to retrieve documents

\paragraph{Limitation(s) and Trade-Off(s)}
% scope: microscope
% info: What are the limitations of the resulting dataset to its consumers, compared to the upstream source(s)? Break down by source type. (Usage Note: Duplicate and complete the following for each source type.)
- The judgement of relevance can be subjective, leading to non-perfect human performance.

\subsubsection{Version and Maintenance}
% info: Fill this next row if this is not the first version of the dataset, and there is no data card available for the first version
\paragraph{First Version}
% scope: periscope
% info: Provide a \textbf{basic description of the first version} of this dataset.
- \textbf{Release date:} 06/2024
- \textbf{Link to dataset:} BRIGHT 1.0: \url{https://huggingface.co/datasets/xlangai/BRIGHT}
- \textbf{Status:} Actively Maintained
- \textbf{Size of Dataset:} 607 MB
- \textbf{Number of Instances:} 1322

\paragraph{Note(s) and Caveat(s)}
% scope: microscope
% info: Summarize the caveats or nuances of the first version of this dataset that may affect the use of the current version. Use additional notes to capture any other relevant information or considerations.
None

\paragraph{Cadence}
% scope: telescope
% info: Select \textbf{one}:
- Daily

\paragraph{Last and Next Update(s)}
% scope: periscope
% info: Please describe the update schedule:
- We have not updated the datasets since release.

\paragraph{Changes on Update(s)}
% scope: microscope
% info: Summarize the changes that occur when the dataset is refreshed. Use additional notes to capture any other relevant information or considerations. (Usage Note: Duplicate and complete the following for each source type.)
N/A

\subsection{Human and Other Sensitive Attributes}

\paragraph{Sensitive Human Attribute(s)}
None

\paragraph{Intentionality}
\begin{itemize}
\item \textbf{Intentionally Collected Attributes}
We only use human-labeled links or tags to find examples or documents, but not directly include human labels.

\item \textbf{Unintentionally Collected Attributes}
None

\end{itemize}

\paragraph{Rationale}
We follow links or tags to find relevant documents or examples.

\paragraph{Source(s)}
None

\paragraph{Methodology Detail(s)}
We follow links or tags to find relevant documents or examples.

\paragraph{Distribution(s)}
N/A

\paragraph{Known Correlations}
\begin{itemize}
    \item \textbf{Attributes:} \texttt{query}, \texttt{gold\_ids}, \texttt{gold\_ids\_long}
    \item \textbf{Description:} The documents corresponding to \texttt{gold\_ids} or \texttt{gold\_ids\_long} are relevant to queries.
    \item \textbf{Impact on dataset use:} It helps evaluate retrieval models in realistic setting.
\end{itemize}

\paragraph{Risk(s) and Mitigation(s)}
\begin{itemize}
\item \textbf{Human Attribute}
None
\end{itemize}

\subsection{Extended Use}

\subsubsection{Use with Other Data}

\paragraph{Safety Level}
\begin{itemize}
    \item Safe to use with other data
\end{itemize}

\paragraph{Known Safe Dataset(s) or Data Type(s)}
The data in BRIGHT benchmark focus on academia-oriented domains, and they should be safe.

\paragraph{Best Practices}
Evaluate retrieval systems on BRIGHT.

\paragraph{Known Unsafe Dataset(s) or Data Type(s)}
None

\paragraph{Limitation(s) and Recommendation(s)}
The judgement of relevance between queries and documents can be subjective, so marginal difference between model evaluation could be ignored, while significant difference gives good signals of model capabilities.

\subsubsection{Forking \& Sampling}

\paragraph{Safety Level}
\begin{itemize}
    \item Safe to form and/or sample
\end{itemize}

\paragraph{Acceptable Sampling Method(s)}
\begin{itemize}
    \item Cluster Sampling
    \item Haphazard Sampling
    \item Multi-stage sampling
    \item Random Sampling
    \item Retrospective Sampling
    \item Systematic Sampling
    \item Weighted Sampling
    \item Unsampled
\end{itemize}

\paragraph{Best Practice(s)}
Although sampling is possible, we recommend not to do it because the size of BRIGHT is not very large.

\paragraph{Risk(s) and Mitigation(s)}
N/A

\paragraph{Limitation(s) and Recommendation(s)}
N/A

\subsubsection{Use in ML or AI Systems}

\paragraph{Dataset Use(s)}
\begin{itemize}
    \item Evaluation
\end{itemize}

\paragraph{Notable Feature(s)}
The intensive reasoning required to retrieve documents.

\paragraph{Usage Guideline(s)}
\begin{itemize}
\item \textbf{Usage Guidelines:} Follow \href{https://github.com/xlang-ai/BRIGHT}{the tutorial} to evaluate retrieval systems.
\item \textbf{Approval Steps:} Steps are \href{https://github.com/xlang-ai/BRIGHT}{here}.

\item \textbf{Reviewer:} We authors review the dataset for publication.
\end{itemize}

\paragraph{Distribution(s)}
The BRIGHT benchmark is for the purpose of evaluation, i.e., all data are in test set.

\paragraph{Known Correlation(s)}
\begin{itemize}
    \item \textbf{Attributes:} \texttt{query}, \texttt{gold\_ids}, \texttt{gold\_ids\_long}
    \item \textbf{Description:} The documents corresponding to \texttt{gold\_ids} or \texttt{gold\_ids\_long} are relevant to queries.
    \item \textbf{Impact on dataset use:} It can help evaluate retrieval systems in more realistic scenarios.
    \item \textbf{Risks from correlation:} The judgement of correlation is by real users, and can be subjective.
\end{itemize}

\paragraph{Split Statistics}
\begin{itemize}
\item Data statistics of \ours
\\\\
\begin{tabular}{lcccccc}
\hline
\textbf{Dataset} & \textbf{\# Q} & \textbf{\# D} & \textbf{\# D+} & \textbf{Q.L.} & \textbf{D.L.} \\ \hline
Biology & 103 & 57,364 & 3.6 & 83.6 & 115.2 \\
Earth Science & 118 & 122,388 & 7.7 & 132.4 & 113.3 \\
Economics & 103 & 50,221 & 8.0 & 120.2 & 181.5 \\
Psychology & 101 & 52,841 & 7.3 & 118.2 & 149.6 \\
Robotics & 101 & 62,198 & 5.5 & 120.6 & 818.9 \\
Stack Overflow & 117 & 101,100 & 7.0 & 704.5 & 478.3 \\
Sustainable Living & 108 & 60,732 & 5.6 & 108.0 & 148.5 \\
LeetCode & 142 & 413,932 & 1.8 & 483.1 & 497.5 \\
Pony & 112 & 7,894 & 22.5 & 98.3 & 102.6 \\
AoPS & 111 & 188,177 & 4.7 & 89.0 & 250.5 \\
TheoremQA & 206 & 188,177 & 3.2 & 117.1 & 250.5 \\ \hline
\end{tabular}
\end{itemize}

For each dataset, we show the number of queries (\# Q) and documents (\# D), the average number of positive documents (\# D+) per example, the average length of queries (Q.L.) and documents (D.L., measured by the GPT-2 tokenizer).

\subsection{Transformations}
\textit{Fill this section if any transformations were applied in the creation of your dataset.}

\subsubsection{Synopsis}
\paragraph{Transformation(s) Applied}
\textit{Select all applicable transformations that were applied to the dataset.}
\begin{itemize}
    \item Data Aggregation
\end{itemize}

\paragraph{Field(s) Transformed}
\textit{Provide the fields in the dataset that were transformed. Use additional notes to capture any other relevant information or considerations.}
\begin{itemize}
    \item \textbf{Transformation Type}
    \begin{itemize}
        \item Field Name | Source \& Target \\
        gold\_ids | links: gold\_ids \\
        gold\_ids\_long | links: gold\_ids\_long
    \end{itemize}
\end{itemize}

\paragraph{Library(ies) and Method(s) Used}
\textit{Provide a description of the methods used to transform or process the dataset. Use additional notes to capture any other relevant information or considerations.}
\begin{itemize}
    \item \textbf{Transformation Type}
    \begin{itemize}
        \item \textbf{Method:} We follow the links or tags to find relevant documents.
        \item \textbf{Platforms, tools, or libraries:} We do not leverage other platforms or tools in transformation.
        \item \textbf{Transformation Results:} We collect 1322 examples that can be used for evaluating retrievers.
    \end{itemize}
\end{itemize}

\subsubsection{Breakdown of Transformations}
We find documents for all instances following the procedure above.

\paragraph{Residual \& Other Risk(s)}
\textit{What risks were introduced because of this transformation? Which risks were mitigated?}
The risk is that the relevance judgment is subjective.

\paragraph{Human Oversight Measure(s)}
\textit{What human oversight measures, including additional testing, investigations and approvals were taken due to this transformation?}
We require human annotators to write down the judgment for relevance and reasoning steps.

\paragraph{Additional Considerations}
\textit{What additional considerations were made?}
None

\paragraph{Cleaning Mismatched Value(s)}
We select high-quality data instances from websites, so there is no further cleaning.

\paragraph{Method(s) Used}
We follow links or tags on the websites.

\paragraph{Comparative Summary}
We do not use incorrect or mismatched values.

\paragraph{Residual \& Other Risk(s)}
N/A

\paragraph{Human Oversight Measure(s)}
The data and notes written down by annotators are reviewed.

\paragraph{Additional Considerations}
None

\paragraph{Anomalies}
We select data from websites, so no anomaly or outlier is excluded.

\paragraph{Method(s) Used}
N/A

\paragraph{Platforms, tools, or libraries:}
N/A

\paragraph{Comparative Summary}
N/A

\paragraph{Residual \& Other Risk(s)}
N/A

\paragraph{Human Oversight Measure(s)}
The data and notes written by annotators are reviewed.

\paragraph{Additional Considerations}
None

\paragraph{Dimensionality Reduction}
N/A

\paragraph{Method(s) Used}
N/A

\textbf{Platforms, tools, or libraries:}
N/A

\paragraph{Comparative Summary}
N/A

\paragraph{Residual \& Other Risks}
N/A

\paragraph{Human Oversight Measure(s)}
N/A

\paragraph{Additional Considerations}
None

\paragraph{Joining Input Sources}
We use StackExchange, LeetCode, TheoremQA, and math competitions.

\paragraph{Method(s) Used}
They are independent splits, so no join is performed.

\paragraph{Comparative Summary}
N/A

\paragraph{Residual \& Other Risk(s)}
N/A

\paragraph{Human Oversight Measure(s)}
N/A

\paragraph{Additional Considerations}
N/A

\paragraph{Redaction or Anonymization}
\textit{Which features were redacted or anonymized?}
N/A

\paragraph{Method(s) Used}
\textit{What methods were used to redact or anonymize data?}
N/A

\paragraph{Comparative Summary}
\textit{Why was data redacted or anonymized using this method over others? Provide comparative charts showing before and after redaction or anonymization process.}
N/A

\paragraph{Residual \& Other Risk(s)}
N/A

\paragraph{Human Oversight Measure(s)}
N/A

\paragraph{Additional Considerations}
N/A

\paragraph{Others (Please Specify)}
\textit{What was done? Which features or fields were affected?}
N/A

\paragraph{Method(s) Used}
N/A

\paragraph{Comparative Summary}
\textit{Why was this method used over others? Provide comparative charts showing before and after this transformation.}
N/A

\paragraph{Residual \& Other Risk(s)}
N/A

\paragraph{Human Oversight Measure(s)}
N/A

\paragraph{Additional Considerations}
N/A

\subsection{Annotations \& Labeling}
\paragraph{Annotation Workforce Type}
\begin{itemize}
    \item Human Annotations (Expert)
    \item Human Annotations (Non-Expert)
\end{itemize}

\paragraph{Annotation Characteristic(s)}
\begin{itemize}
    \item \textbf{Annotation Type} | \textbf{Number} \\
    Total number of annotations | 1322
\end{itemize}

\paragraph{Annotation Description(s)}
\textit{Provide descriptions of the annotations applied to the dataset. Include links and indicate platforms, tools or libraries used wherever possible. Use additional notes to capture any other relevant information or considerations.}
\begin{itemize}
    \item \textbf{Description:} Description of annotations (labels, ratings) produced. Include how this was created or authored. We follow links/tags to find relevant documents.
    \item \textbf{Link:} N/A
    \item \textbf{Platforms, tools, or libraries:} N/A
\end{itemize}

\paragraph{Annotation Distribution(s)}
\begin{itemize}
    \item \textbf{Dataset | number} \\
    Biology | 103 \\
    Earth Science | 118 \\
    Economics | 103 \\
    Psychology | 101 \\
    Robotics | 101 \\
    Stack Overflow | 117 \\
    Sustainable Living | 108 \\
    LeetCode | 142 \\
    Pony | 112 \\
    AoPS | 111 \\
    TheoremQA | 206
\end{itemize}
Distribution of data splits in each domain.

\paragraph{Annotation Task(s)}
    \begin{itemize}
        \item \textbf{Task description \& instructions:}
        In this section, we describe the instructions for annotators to collect data in BRIGHT.
        \begin{itemize}
            \item StackExchange
            \begin{itemize}
                \item Browse posts from the newest to the oldest.
                \item Discard posts without an answer accepted by the user or obtains more than 5 votes.
                \item Discard answers of posts without URL links.
                \item For each link in the answer, write down the answers to: (1) why are the document and the post relevant; (2) what is the reasoning required to understand the relevance between the post and the document. If these answers are not possible, discard the link.
                \item Use LLMs (e.g., ChatGPT, Claude, etc.) to generate post keywords, or use the post title to search for web pages with large keyword or semantic overlap in Google. Search for at most 5 negative web pages per query.
                \item Split every web page into small passages either by two newline symbols, "\#" in markdown files or fixed-length tokens.
            \end{itemize}
            \item TheoremQA
            \begin{itemize}
                \item In TheoremQA, the main task for the annotator is to check if the GPT-4 rewritten questions are valid.
                \item The specific instructions are as follows:
                \begin{itemize}
                    \item Read the rewritten question and determine if it is solvable.
                    \item If it is solvable, read the original question and solution, and determine if the rewritten question is consistent with the original question. That is, the same reasoning steps and the final answer should hold.
                    \item If it is also consistent, mark the question as valid, and make any minor edits to the problem statement (e.g., to improve grammar or fluency) as you see fit.
                    \item If it is not solvable or not consistent, read the original question and solution, and correct the rewritten question if possible. If not, then discard the problem.
                \end{itemize}
            \end{itemize}
            \item AoPS
            \begin{itemize}
                \item In AoPS, annotators are tasked to find questions from the AoPS Wiki and record the problems:
                \item Browse through the AoPS Wiki and find topic/category pages (example 1, example 2).
                \item Look through each page and find pages specific theorems or techniques that can be used to solve problems. The page should link to at least two competition problems (example 1, example 2).
                \item Record the links of both the theorem/technique as well as the problem pages.
                \item The annotators are assigned a category to look for theorems to avoid overlaps, and the categories are {algebra, geometry, calculus, probability, number theory, other}.
                \item After all links are collected, we use a web scraper to collect the problem statement and solutions, and we manually check the quality of the scraped data.
            \end{itemize}
            \item LeetCode
            \begin{itemize}
                \item In LeetCode, annotators determine whether a question is grounded in real-world concepts. We give a similar instruction to the annotator as to GPT-4:
                \begin{itemize}
                    \item Read the problem statement carefully.
                    \item Categorize the question into one of three categories: 0: The question is not grounded in any real-world concepts. The description only uses coding-specific terms, such as "linked list", "binary search", "palindrome", "sorting", etc., 1: The question is not grounded in any real-world concepts or real-world concepts that are commonly used in the context of coding, such as needle in a haystack, strings/words, or a spiral matrix.3, : The question is grounded in real-world concepts that are not commonly used in the context of coding, such as building height, planting trees, or games. It may still use some code-specific terms to specify the data structure involved.
                \end{itemize}
            \end{itemize}
        \end{itemize}
    \item \textbf{Methods used:} Basically, we follow links/tags to find documents.
    \item \textbf{Inter-rater adjudication policy:} Reviewers annotate where the pairing of queries and documents is not convincing.
    \item \textbf{Golden questions:} N/A
\end{itemize}

\subsubsection{Human Annotators}
\paragraph{Annotator Description(s)}
\begin{itemize}
    \item \textbf{Annotation Type}
    \begin{itemize}
        \item \textbf{Task type:} Annotate StackExchange data
        \item \textbf{Number of unique annotators:} 3
        \item \textbf{Expertise of annotators:} Both experts and non-experts
        \item \textbf{Description of annotators:} PhD students in computer science, biology, environment, etc.
        \item \textbf{Language distribution of annotators:} They all speak fluent English.
        \item \textbf{Geographic distribution of annotators:} They come from Asia.
        \item \textbf{Summary of annotation instructions:} Follow links to find documents with filtering.
        \item \textbf{Summary of gold questions:} N/A
        \item \textbf{Annotation platforms:} Google sheets
        \item \textbf{Additional Notes:} N/A
    \end{itemize}
\end{itemize}

\paragraph{Annotator Task(s)}
\begin{itemize}
    \item \textbf{Task Type}
    \begin{itemize}
        \item \textbf{Task description:} Annotate math and code data
        \item \textbf{Task instructions:} Follow tags to find similar problems/questions
        \item \textbf{Methods used:} Follow tags annotated by websites
        \item \textbf{Inter-rater adjudication policy:} The data is reviewed.
        \item \textbf{Golden questions:} N/A
        \item \textbf{Additional notes:} N/A
    \end{itemize}
\end{itemize}

\paragraph{Language(s)}
\begin{itemize}
    \item \textbf{Annotation Type}
    \begin{itemize}
        \item 100\% English
    \end{itemize}
\end{itemize}

\paragraph{Location(s)}
\begin{itemize}
    \item \textbf{Annotation Type}
    \begin{itemize}
        \item Asia [50 \%]
        \item US [50 \%]
    \end{itemize}
\end{itemize}

\paragraph{Gender(s)}
\begin{itemize}
    \item \textbf{Annotation Type}
    \begin{itemize}
        \item Male [80 \%]
        \item Female [20 \%]
    \end{itemize}
\end{itemize}

\subsection{Validation Types}
\subsubsection{Method(s)}
\textit{Select all applicable:}
\begin{itemize}
    \item Code/cross-reference Validation
\end{itemize}

\subsubsection{Breakdown(s)}
\begin{itemize}
    \item \textbf{Validation Type}
    \begin{itemize}
        \item \textbf{Number of Data Points Validated:} 1322
        \item \textbf{Fields Validated:} All fields in data are validated.
    \end{itemize}
\end{itemize}

\paragraph{Description(s)}
\begin{itemize}
    \item \textbf{Validation Type}
    \begin{itemize}
        \item \textbf{Method:} Describe the validation method here. Include links where necessary. We require annotators to write the logic to determine the relevance between queries and documents. The reviewers not only check the data, but also annotators' notes.
        \item \textbf{Validation Results:} Over 90\% of annotation passes peer review, and we discard the rest.
    \end{itemize}
\end{itemize}

\subsubsection{Description of Human Validators}
\paragraph{Characteristic(s)}
\textit{Provide characteristics of the validator pool(s). Use additional notes to capture any other relevant information or considerations.}
\begin{itemize}
    \item \textbf{Validation Type}
    \begin{itemize}
        \item Unique validators: 8
        \item Number of examples per validator: 300
        \item Average cost/task/validator: N/A
        \item Training provided: N
        \item Expertise required: N
    \end{itemize}
\end{itemize}

\paragraph{Description(s)}
\begin{itemize}
    \item \textbf{Validation Type}
    \begin{itemize}
        \item \textbf{Validator description:} Validators are domain experts, e.g., PhD students from the corresponding domains.
        \item \textbf{Training provided:} We do not provide training, but verify that the annotators, reviewers are qualified.
        \item \textbf{Validator selection criteria:} We have a test containing verified examples. An annotator is qualified if they can work out these examples.
        \item \textbf{Training provided:} N/A
    \end{itemize}
\end{itemize}

\paragraph{Language(s)}
\begin{itemize}
    \item \textbf{Validation Type}
    \begin{itemize}
        \item English [100 \%]
    \end{itemize}
\end{itemize}

\paragraph{Location(s)}
\begin{itemize}
    \item \textbf{Validation Type}
    \begin{itemize}
        \item Asia [60 \%]
        \item US [40 \%]
    \end{itemize}
\end{itemize}

\paragraph{Gender(s)}
\begin{itemize}
    \item \textbf{Validation Type}
    \begin{itemize}
        \item Male [70 \%]
        \item Female [30 \%]
    \end{itemize}
\end{itemize}

\subsection{Sampling Methods}
\subsubsection{Method(s) Used}
\textit{Select all applicable methods used in the creation of this dataset:}
\begin{itemize}
    \item Unsampled
\end{itemize}

\subsubsection{Characteristic(s)}
N/A

\subsubsection{Sampling Criteria}
N/A

\subsection{Known Applications \& Benchmarks}
\subsubsection{ML Application(s)}
\textit{Provide a list of key ML tasks that the dataset has been used for.}
\textit{Usage Note: Use comma-separated keywords.}
Retrieval evaluation

\subsubsection{Evaluation Result(s)}
\begin{itemize}
    \item SFR-Embedding-Mistral 17.8
    \item \textbf{Model Card:} \url{https://huggingface.co/Salesforce/SFR-Embedding-Mistral/tree/main}
    \item \textbf{Evaluation Results:}
    \begin{itemize}
        \item nDCG@10: 17.8
    \end{itemize}
\end{itemize}

\subsubsection{Evaluation Process(es)}
We write python scripts to run retrieval models on BRIGHT.

\paragraph{Description(s) and Statistic(s)}
\begin{itemize}
    \item SFR-Embedding-Mistral
    \begin{itemize}
        \item \textbf{Model Card:} \url{https://huggingface.co/Salesforce/SFR-Embedding-Mistral/tree/main}
        \item \textbf{Model Description:} The best-class retrieval model trained from mistral-7b.
        \begin{itemize}
            \item Model Size: 7.11B
            \item Model Weights: 7.11B
            \item Model Layers: 32
            \item Latency: 2s
        \end{itemize}
    \end{itemize}
\end{itemize}

\subsubsection{Expected Performance and Known Caveats}
\begin{itemize}
    \item Claude-3 + BM25
    \begin{itemize}
        \item \textbf{Expected Performance:} Surpasses results obtained without using LLMs.
        \item \textbf{Known Caveats:} The inference of LLMs can be expensive.
    \end{itemize}
\end{itemize}

\subsection{Terms of Art}
\subsubsection{Concepts and Definitions referenced in this Data Card}
\paragraph{BRIGHT}
\begin{itemize}
\item \textit{Definition: The name of this benchmark}
\item \textit{Source:}\url{https://huggingface.co/datasets/xlangai/BRIGHT}
\item \textit{Interpretation: N/A}
\end{itemize}

\subsection{Reflections on Data}
We believe that BRIGHT paves the way for future research on retrieval systems in more realistic and challenging settings.



==> texts/appendices/misc.tex <==

\section{Dataset Documentation}
\input{texts/appendices/datadoc}

\section{Other Dataset Information}
\subsection{Dataset URLs}
\textbf{URL to benchmark.} The benchmark URL can be found here: \href{https://huggingface.co/datasets/xlangai/BRIGHT}{link}

\textbf{URL to Croissant metadata.} The Croissant metadata URL can be found here: \href{https://huggingface.co/api/datasets/xlangai/BRIGHT/croissant}{link}

\subsection{Author Statement \& License Information}
 We the authors bear all responsibility in case of violation of rights. We provide the license information for the data we used to construct \ours{}:
 
 \textbf{StackExchange.} The data is publicly available and licensed under Creative Commons Attribution-ShareAlike license as follows:
\begin{itemize}
    \item Content contributed before 2011-04-08 (UTC) is distributed under the terms of CC BY-SA 2.5.
    \item Content contributed from 2011-04-08 up to but not including 2018-05-02 (UTC) is distributed under the terms of CC BY-SA 3.0.
    \item Content contributed on or after 2018-05-02 (UTC) is distributed under the terms of CC BY-SA 4.0.
\end{itemize}
Please find detailed information on the license at \url{https://stats.stackexchange.com/help/licensing}.

\textbf{LeetCode.} According to LeetCode's \href{https://leetcode.com/terms/}{Terms of Service}, the data on the platform is owned by the LeetCode Service. Following \cite{hendrycks2021measuring} and \cite{jain2024livecodebench}, we scrape the problem statement, solutions, test cases, similar problem annotations, and topics from the LeetCode website. We do not store any user data or any other proprietary information from the LeetCode platform. We abide by Fair Use §107: “the fair use of a copyrighted work, including such use by ... scholarship, or research, is not an infringement of copyright”, where fair use is determined by “the purpose and character of the use, including whether such use is of a commercial nature or is for nonprofit educational purposes” and “the effect of the use upon the potential market
for or value of the copyrighted work.”

\textbf{Pony.} Pony is licensed under apache-2.0 License according to its \href{https://huggingface.co/datasets/xlangai/arks_data}{HuggingFace dataset card}.

\textbf{TheoremQA \& AoPS.} TheoremQA is licensed under MIT License according to its \href{https://huggingface.co/datasets/TIGER-Lab/TheoremQA}{HuggingFace dataset card}. AoPS does not provide license information according to its \href{https://artofproblemsolving.com/wiki/index.php/AoPS_Wiki:Copyright}{Copyright statement}. 

\subsection{Hosting and maintenance.} We have a dedicated GitHub page to host the leaderboard (\url{https://brightbenchmark.github.io/}) while data and codebase will be hosted on Huggingface (\url{https://huggingface.co/datasets/xlangai/BRIGHT}) and GitHub (\url{https://github.com/xlang-ai/bright}). We are committed to performing major maintenance on \ours{} every 3-6 months.



==> texts/checklist.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes%{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{In Appendix~\ref{app:limitation}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{In Appendix~\ref{app:social_impact}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code, data, and instructions will be in the supplemental materials}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{In Appendix~\ref{app:experiment_details}}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNo{Our experiments on open-sourced models are deterministic, and it is expensive to run with large language models like GPT-4 multiple times.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{In Appendix~\ref{app:machines}}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We establish the code and data from scratch, and cite every model evaluated in this paper.}
  \item Did you mention the license of the assets?
    \answerYes{In Appendix~\ref{app:modelinstructions}}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{We create a new benchmark and code base, which will be in the supplementary materials}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{All the models used in the paper allow research use}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{In Appendix~\ref{app:sensitive}}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerYes{In Appendix~\ref{app:annotator_instruction}}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}
